Making transport more robust and interpretable by moving data through a small number of anchor points

Optimal transport (OT) is a widely used technique for distribution alignment, with applications throughout the machine learning, graphics, and vision communities. Without any additional structural assumptions on trans-port, however, OT can be fragile to outliers or noise, especially in high dimensions. Here, we introduce a new form of structured OT that simultaneously learns low-dimensional structure in data while leveraging this structure to solve the alignment task. Compared with OT, the resulting transport plan has better structural interpretability, highlighting the connections between individual data points and local geometry, and is more robust to noise and sampling. We apply the method to synthetic as well as real datasets, where we show that our method can facilitate alignment in noisy settings and can be used to both correct and interpret domain shift.

==> alg2.tex <==
\vspace{-2mm}
\subsection{Algorithms}
\vspace{-2mm}
In this section, we will develop our main approach for finding a factorization of the transport plan that can be decomposed to reveal structure in the source and target datasets. Our approach consists of two main ingredients: (i) a method that can find a transport plan given a set of anchors, and (ii) an approach to find anchors at the same time as we are solving (i). Now we step through algorithms for solving both of these.

%two main algorithms. (1) We assume we know the anchors, to establish baseline conditions. (2) Unknown anchors. \eva{@henry - please give reader a sense of where you are going w/ algorithm design. What is flow of method when you put it together later?}

\vspace{-2mm}
\subsubsection*{Alg.~1: What if the anchors are known?}
\vspace{-2mm}

While our goal is to build an algorithm that can both find anchors and also transport mass through them, to start, we will assume that the anchors are known. This will become a sub-routine of our full algorithm. We assume that the anchors are supported on finite locations, i.e., ${\cal{Z}}_x=\{z^x_1,\dots,z^x_{k_1}\}$ and ${\cal{Z}}_y=\{z^y_1,\dots,z^y_{k_2}\}$.
%This case naturally arises when we have accessed to side information like a cluster label, or 
The \alg is a linear programming problem, but the computation could be slow when the number of data points is large. For accelerations, we add the entropy regularizations to the three transport terms in Def. \ref{def1}. This produces three kernels $\mathbf{K}_x,\mathbf{K}_z,\mathbf{K}_y$ from the cost matrices $\mathbf{C}_{X,Z},\mathbf{C}_Z,\mathbf{C}_{Z,Y}$, and transforms our  optimization into,
\begin{align}\label{cost1for}
    &\min_{\mathbf{u}_z\in\Sigma_{k_1},\mathbf{v}_z\in\Sigma_{k_2}}\min_{(\mathbf{P}_x,\mathbf{P}_z,\mathbf{P}_y)\in{\cal{G}}} \epsilon(\text{KL}(\mathbf{P}_x\|\mathbf{K}_x)+\text{KL}(\mathbf{P}_z\|\mathbf{K}_z)+\text{KL}(\mathbf{P}_y\|\mathbf{K}_y)),\\
    \text{where }& {\cal{G}}=\{(\mathbf{P}_x,\mathbf{P}_y,\mathbf{P}_z):\mathbf{P}_x\mathbbm{1} =\mu,\mathbf{P}^T_x\mathbbm{1}=\mathbf{u}_z,\mathbf{P}_z\mathbbm{1} = \mathbf{u}_z,\mathbf{P}_z^T\mathbbm{1} =\mathbf{v}_z,\mathbf{P}_y\mathbbm{1}=\mathbf{v}_z,\mathbf{P}^T_y\mathbbm{1}=\nu\}. \nonumber
\end{align}
The constraint set is defined by affine functions of variables, hence we can solve this problem using an iterative Bregman projection strategy \citep{benamou2015iterative}.
The procedure is described in Algorithm \ref{alg:1}. 
It involves applying Bregman projections iteratively to the three terms in the objective: projection of first term in Line 5, the second term in Lines 6-8, and the last term in Line 9. We defer the detailed derivation to the Appendix.

%####### ALGORITHM 
\input{alg}

\vspace{-2mm}
\subsubsection*{Alg.~2: What if the anchors are unknown?}
\vspace{-2mm}
Now we extend the approach in the previous subsection to optimize the anchor locations at the same time. 
%We see that the previous algorithm becomes a subroutine of our overall approach described in this section.
We consider Euclidean space $\Omega=\mathbb{R}^d$ and the anchors are free to move in the entire space, i.e., ${\cal{Z}}_x={\cal{Z}}_y=\Omega$.
In order to optimize the locations, we rewrite the objective of \alg in terms of function of them.
\eva{@Henry-dont you need this notation earlier? X,Y,Z}Let $\mathbf{X}=[\mathbf{x}_1,\dots,\mathbf{x}_n]$, $\mathbf{Y}=[\mathbf{y}_1,\dots,\mathbf{y}_m]$ be the data matrices, and $\mathbf{Z}_x=[\mathbf{z}^x_1,\dots,\mathbf{z}^x_{k_1}]$,  $\mathbf{Z}_y=[\mathbf{z}^y_1,\dots,\mathbf{z}^y_{k_2}]$ be anchor matrices with columns being the anchors to the source and the target, respectively. The objective \eva{Which objective?} is equal to,
\begin{align}\label{xform}
    \text{tr}\left(\mathbf{Z}_x^T(\mathbf{M}_x+\mathbf{M}_y)\mathbf{Z}_x\text{diag}(\mathbf{u}_z)\right)+\text{tr}\left(\mathbf{Z}_y^T(\mathbf{M}_y+\mathbf{M}_z)\mathbf{Z}_y\text{diag}(\mathbf{v}_z)\right)\nonumber\\
    -2\text{tr}\left(\mathbf{P}_x^T\mathbf{X}^T\mathbf{M}_x\mathbf{Z}_x\right)-2\text{tr}\left(\mathbf{P}_z^T\mathbf{Z}_x^T\mathbf{M}_z\mathbf{Z}_y)-2\text{tr}(\mathbf{P}_y^T\mathbf{Z}_y^T\mathbf{M}_y\mathbf{Y}\right).
\end{align}
We get the first-order stationary point by setting the gradient of (\ref{xform}) with respect to $\mathbf{Z}_x$ and $\mathbf{Z}_y$, which results in the closed-form formula,
\begin{align}\label{cenfor}
    \begin{bmatrix}\text{vec}(\mathbf{Z}_x^*)\\\text{vec}(\textbf{Z}_y^*)
    \end{bmatrix}=\begin{bmatrix}
\text{diag}(\mathbf{u}_z)\otimes (\mathbf{M}_x+\mathbf{M}_z) & \mathbf{P}_z\otimes \mathbf{M}_z\\
-\mathbf{P}_z^T\otimes \mathbf{M}_z & \text{diag}(\mathbf{v}_z)\otimes (\mathbf{M}_y+\mathbf{M}_z) 
\end{bmatrix}^{-1}\begin{bmatrix}(\mathbf{P}_x^T\otimes \mathbf{M}_x)\text{vec}(\mathbf{X})\\(\mathbf{P}_y\otimes \mathbf{M}_y)\text{vec}(\mathbf{Y})
    \end{bmatrix},
\end{align}
where vec denotes vectorization operator converting a matrix to a column vector.
Combining Algorithm \ref{alg:1} with (\ref{cenfor}), we propose a Floyd-type algorithm by alternatively optimizing transport plans $(\mathbf{P}_x,\mathbf{P}_y,\mathbf{P}_z)$ and the anchors $(\mathbf{Z}_x,\mathbf{Z}_y)$. The complete algorithm is summarized in Algorithm \ref{alg:2}. 

%Recall the definition of the Mahalanobis distance, $\|\x-\y\|_{\mathbf{M}}^2:=(\x-\y)^T{\mathbf{M}}(\x-\y)$, where ${\mathbf{M}}$ is some positive semi-definite matrix. This class of cost functions has recently gained substantial interests due to its key role leading to robust OT \citep{paty2019subspace,dhouib2020swiss}. Denote ${\mathbf{M}}_x$, ${\mathbf{M}}_z$, ${\mathbf{M}}_y$ be the associated Mahalanobis matrices correspond to $\mathbf{C}_{X,Z}$, $\mathbf{C}_Z$, and $\mathbf{C}_{Z,Y}$, respectively. 
                                                  

==> discussion.tex <==
\vspace{-1mm}
\section{Discussion}\label{sec:discussion}
\vspace{-2mm}
In this paper, we introduced a new algorithm for Bayesian optimization that leverages known modular structure in an otherwise black-box system to minimize the overall cost required for global optimization. To do this, we introduced a new notion of regret, \textit{movement augmented regret}, that captures the notion of trying to minimize the number of changes to variables in early modules of a system.
%This addressed the issue of how to incorporate structural information into our optimization design. 
We designed an algorithm to minimize the movement augmented regret and demonstrated that our method performs well both in theory and in practice. In our analysis, we showed that \alg~ achieves sublinear movement regret. In practice, we showed that our method outperforms other standard approaches in both synthetic datasets and in a brain mapping application. Thus, our results demonstrate that \alg~ not only can be used to achieve good performance for global optimization but can also be used to reduce the optimization cost of structured black-box systems.

\vspace{-3mm}
\paragraph{Broader impacts:} This paper addresses a real-world problem of system optimization that is encountered in a variety of scientific disciplines. Increasingly, as we expand the size of datasets in these different domains, we need automated solutions to apply advanced machine learning systems to new datasets and re-optimize  systems in an end-to-end manner. Here, we showed how to leverage structure in such systems to inspire the design of a new black-box optimization approach. We demonstrated its application in a relatively simple neuroscience application; however, this method provides a general approach that can be used in a number of scientific domains and make major impacts in advancing healthcare and science.



==> experiment.tex <==
\begin{figure*}[t!]
\centering
   \includegraphics[width=\textwidth]
   {fig2_ver131.png}
   
   \vspace{-1mm}
\caption{\footnotesize {\em Results on synthetic datasets and a brain mapping example.} 
In (A-D), we compare 
\alg~with other BO algorithms on synthetic functions in a two module setting with a cost ratio of $10$ to 1. In (A-B), we show the results for two different synthetic functions (Hartmann, Rastrigin) and in (C), we investigate the impact of dimension across modules. In (D), the decrease rate verifies our theory that \alg~can effectively diminish the movement regret. In (E), we show the performance when the cost ratio equals one, using the same function as in (A). (F) explores the three module setting, where the costs are $=[40,10,1]$. In (G-H), we depict a brain mapping pipeline consisting of three modules. 
(H) shows the results for the full pipeline and (G) depicts a simplified example where we remove the first module.}
\label{fig:syn}
    \vspace{-3mm}
\end{figure*}


\vspace{-3mm}
\section{Experiments}\label{sec:exp}
\vspace{-2mm}
In this section, we evaluate the performance on two different tasks and compare with other methods for BO. First, we test \alg~on benchmark synthetic functions used in other studies \cite{vellanki2017process,kirschner2019adaptive}. Following this, we study \alg's performance on an  neuroscience application where multiple modules are jointly optimized to maximize end-to-end performance.

\vspace{-3mm}
\paragraph{Synthetic datasets:}
For synthetic benchmarks we selected the 6D Hartmann, 6D Rastrigin, and 6D Griewank  functions, as well as the 8D Ackley function. To simulate a $2$-module scenario, we partition the dimension space of the modules to be $[3,3]$, $[3,3]$, $[4,2]$, and $[6,2]$, respectively. 
To emphasize the the effect of accumulation of cost in early stages of processing, we set the cost ratio between the first and second module of 10 to 1. The sampling noise $\epsilon$ is assumed to be independent Gaussian with standard deviation $0.01$. 
For simplicity, we used the squared exponential kernel and initialized it using $15$ random samples before starting the inference procedure.
In our experiments, the functions are normalized by their maximized absolute value for clear comparisons,  the regularization parameter is fixed to $\lambda=0.1$, the UCB parameter is set each iteration as $\beta_t=0.2D\log 2t$, and the learning rate is set to $\eta = 1$. For construction of MSET, we test on the simplest case where $d_i=1$ and partition the variable space in each module into 2 sets aligned with a random coordinate. In practice, we found some adaptive strategies could boost the performance (see Supp. B.2 for further details). The curves on synthetic data and real data were computed by averaging across $100$ and $20$ simulations, respectively, to provide information about the variability across different random initializations.

We compared \alg~ with common baselines GP-UCB\cite{Srinivas:2010:GPO:3104322.3104451}, GP-EI\cite{movckus1975bayesian}, Max-value entropy search \cite{wang2017max},  random sampling, and three cost-aware strategies: EIpu \cite{snoek2012practical}, CA-MOBO \cite{abdolshah2019cost}, and CArBO \cite{lee2020costaware}. To adapt the cost-aware strategies to our setting, we set the sampling cost associated with switching variables in modules. To start, we tested the methods on two synthetic functions ({\bf Figure~\ref{fig:syn}A-B}) (Supp. B.3 provides results for two additional synthetic functions). Empirically we find that in most of the synthetic cases tested, \alg~performs similarly to other methods early on, but with further iterations, \alg~ starts to outperform the alternatives. This could be explained by inaccurate estimation of function at early stages, and the fact that aggressive input changes could outperform the more conservative or lazy strategy used in \alg. However, as more samples are gathered, \alg~demonstrates more power in terms of its cost efficiency by being lazy in variable switching. The traditional cost-aware strategies do not perform well because they use static strategies to treat the dynamic \textit{switching} costs 
and ignore the effect of \textit{modular structure}. We also complement our finding by verifying the theory. We use 6D Hartmann function to study the convergence of \alg~ in terms of the cumulative movement regret, by computing the averaged movement regret $R_T^+/T$ as a function of time horizon $T$ ({\bf Figure.~\ref{fig:syn}D}). \alg~ has minimal regret and cost-aware methods have intermediate results between non-cost-aware strategies and ours. These results point to the superiority of \alg~ over direct adaptation from traditional cost-aware strategies. 

We investigate how modular structure affects our algorithm from three different angles: variable dimension, cost ratio, and number of modules.
To find out  answers to these questions, we conduct a number of experiments. First, we study the impact of dimension by splitting the variables in the Ackley 8D into three different configurations ($[2,6]$, $[4,4]$, and $[6,2]$) ({\bf Figure~\ref{fig:syn}C}). We find that our method has consistent performance among the different variable splits, with some degradation as the complexity of the first module increases, which suggests that aggressive switching can be essential when optimizing a module is hard. 
Second, we examine the impact of the relative cost of modules. For this purpose, we conduct the same experiment as in (A) but change the cost ratio to be 1:1 ({\bf Figure~\ref{fig:syn}E}). In this case, existing cost-aware methods have the best performance while \alg~ attains comparative results. It suggests that our algorithm can be even more beneficial in the asymmetric cost setting. Third, we explore a 3-module problem, where the Ackley 8D test function is divided into  $[2,2,4]$ dimensions and the cost is set to $[40,10,1]$, respectively across modules ({\bf Figure~\ref{fig:syn}F}). We observe that \alg~ outperforms alternatives by a large amount, which amplifies the advantage of \alg~ when the system is comprised of more modules. 

\vspace{-2mm}
\paragraph{Optimizing a multi-stage neuroimaging pipeline:}
Segmentation and identification of neural structures of interest (e.g., cell bodies, axons, or vasculature) is an important problem in connectomics and other applications of brain mapping \cite{helmstaedter2013connectomic,oh2014mesoscale}. When dealing with large datasets, transfer can be challenging and thus workflows must be re-optimized for each new dataset \cite{johnson2019toward}.  Here, we consider the optimization of a a relatively common three stage brain mapping pipeline, consisting of a pre-processing (image enhancement via denoising and contrast normalization), semantic segmentation  for pixel-level prediction (via a U-net architecture), and a post-processing operation (to reconstruct a 3D volume and detect objects therein). To optimize this pipeline, we use a publicly available X-ray microCT dataset \cite{prasad2019mapping} to set up the experiments in both a two-module (no pre-processing) and  full three-module version of the pipeline (details of search space for each module in Supp. B.1.) In our experiments, we define the cost to be the aggregate recorded clock time for generating an output after changing a variable in a specific module, which were $326.059 \pm 128.390$ sec (pre), $324.539 \pm 128.367$ sec (U-net), and $54.773 \pm 0.894$ sec (post). To test \alg~on the problem, we gathered a data set consisting of $606,000$ combinations of hyperparameters by exhaustive search. The best set of hyperparameters in this case achieved an f1-score of $77.129\%$.
In the two-module case ({\bf Figure~\ref{fig:syn}G}), we observed a transition effect; when enough cost has been spent, \alg~starts to increase its gap in performance over other methods. In the three-module case ({\bf Figure~\ref{fig:syn}H}) the advantage is even more pronounced, where the transition happens earlier. 
Quantitatively it shows that to get close to the optimum (within 5\%), \alg~can achieve this result in only 25\% of the time required by the best alternative approach (1.4 vs. 5.6 hours).


==> figure3.tex <==
\begin{figure*}[t!]
    \centering
    \subfloat{\includegraphics[height=0.22\textwidth]
   {imgs/mnist_lot_graph.png}}
   \subfloat{\includegraphics[height=0.22\textwidth]
   {imgs/usps_graph.png}}\\

    \subfloat{\includegraphics[height=0.14\textwidth]
   {imgs/sankey_mnist.png}}
   \subfloat{\includegraphics[height=0.14\textwidth]
   {imgs/sankey_usps.png}}\\
   
    \subfloat{\includegraphics[width=0.25\textwidth]
   {imgs/cm_before.png}}
   \subfloat{\includegraphics[width=0.25\textwidth]
   {imgs/cm_lot.png}}
    \subfloat{\includegraphics[width=0.35\textwidth]
   {imgs/placeholder_digits.png}}
    
    \caption{\footnotesize {\bf{\em  Concept drift and domain adaptation in handwritten digit recognition.}} In this example, we train an encoder on MNIST and then study alignment in two cases: (i) the source is a noisy (masked) version of the MNIST dataset, and (ii) USPS digits are passed instead of the MNIST data, which represents an example of naturally occurring domain shift. Top: visualization of transport plans obtained via our method and OT. This highlights the interpretability of our approach. Bottom: The confusion matrices and visualization of point-to-point correspondences obtained in both examples. \mehdi{Sankey plots are still a WIP. Not all these plots will be included. Just including all versions so we can decide}   \label{fig:mnist}}
\end{figure*}




==> intro_new2.tex <==
\section{Introduction}\label{sec:intro}
%Optimal transport (OT) \cite{villani2008optimal} is 
Optimal transport (OT) \cite{villani2008optimal} is a widely used technique for distribution alignment that finds a mapping between two distributions by transporting mass to match the two distributions. Due to its flexibility and new tools for finding efficient transport plans, OT has found applications in many diverse areas of machine learning, with examples in domain adaptation \cite{courty2014domain,flamary2016optimal}, generative modeling \cite{martin2017wasserstein,tolstikhin2017wasserstein} 
document retrieval \cite{kusner2015word}, computer graphics \cite{solomon2014earth,solomon2015convolutional,bonneel2016wasserstein}, and computational neuroscience \cite{gramfort2015fast,lee2019hierarchical}. While the ground metric used in \ot can be used to impose geometric structure into transport, without any additional 
assumptions, \ot can be fragile to outliers or noise, especially in high dimensions. 
To overcome this issue, it can be helpful to incorporate additional structure into transport to improve alignment or make transport more robust to noise. Examples of structured \ot approaches include the use of hierarchical or cluster consistency \cite{lee2019hierarchical,yurochkin2019hierarchical,xu2020learning},  partial class information \cite{flamary2016optimal,courty2014domain}, submodular cost functions \cite{alvarez2018structured}, or through low-rank transportation constraints \cite{forrow2019statistical, altschuler2019massively}.
Because of the difficulty of incorporating structure into optimal transport, many \ot methods need low-dimensional structure in data to be specified in advance (e.g., estimated clusters or supervised labels).  

To simultaneously learn low-dimensional structure in data and use it in transport, \citet{forrow2019statistical} proposes a statistical approach that builds a factorization of the transport plan to regularize the rank of OT. 
After factorization, transport from a source to target distribution can be visualized as the flow of mass through a small number of anchors (hubs), which serve as relay stations through which transportation must pass (see Figure~\ref{fig:motivation}, a vs.~b). 
Although this idea of moving data through anchors is appealing, in previous work, the anchors used to constrain transport are {\em shared} by the source and target. As a result, when the source and target contain different structures or experience domain shift \cite{courty2014domain}, shared anchors may not provide an adequate representation for both domains simultaneously.

In this work, we propose a new structured transport approach called Latent Optimal Transport (\alg\hspace{-1mm}). The main idea behind \alg is to factorize the transport plan into three components, where mass is moved: (i) from individual source points to source anchors, (ii) from the source anchors to target anchors, and (iii) from target anchors to individual target points (Figure~\ref{fig:motivation}c-d).
The intermediate transport plan captures the high-level structural similarity between the source and target, while the outer transport plans cluster data in their respective spaces.
By allowing the source and target to have different anchors and aligning the latent spaces of the anchors, the mapping between datasets can be more easily interpreted.
%In both theoretical and empirical studies, we show that \alg regularizes the rank of transport and has the effect of making transport more robust to different perturbations and outliers. 


\begin{figure*}
     \centering

     \subfloat[][\footnotesize{\ot}]{\includegraphics[width=.24\textwidth]{imgs/fig11.png}\label{fig:illus1}\vspace{-3mm}}
     \subfloat[][\footnotesize{\fc}]{\includegraphics[width=.24\textwidth]{imgs/fig14.png}\vspace{-3mm}}
     \subfloat[][\footnotesize{\alg(4,4)}]{\includegraphics[width=.24\textwidth]{imgs/fig12.png}\label{fig:illus2}\vspace{-3mm}}
     \subfloat[][\footnotesize{\alg(8,4)}]{\includegraphics[width=.24\textwidth]{imgs/fig13.png}\label{fig:illus3}\vspace{-3mm}}
     \caption{\footnotesize{{\bf \em  Comparisons of transport plans obtained for different methods applied to clustered data after domain shift}. Here, we visualize the connection between source (blue) $x$  and its estimated transportation in target (red) $\hat{y}=\argmax_y p(y|x)$. From left to right, we show the standard \ot plan (a) and the factored coupling (\url{FC}) approach (b). In (c-d), we show \alg with 4 anchors in the source and target (c), as well as 8 in source and 4 in target (d). }
     \label{fig:motivation}\vspace{-4mm}}
\end{figure*}

Specifically, our contributions are as follows. (i) We introduce \alg\hspace{-1mm}, a new form of structured transport, and propose an efficient algorithm that solves our proposed objective (Section \ref{sec:formulation}), (ii)
Theoretically, we show that \alg can be interpreted as factored-form relaxation to an OT problem,
and from a statistical point-of-view, it overcomes the curse of dimensionality in terms of the sampling rate (Section \ref{sec:analysis}),
(iii) We study the robustness of the approach to noise, sampling, and various data perturbations when applied to both synthetic data and domain adaptation problems in computer vision  (Section~\ref{sec:experiment}).

